Recognizing hyperelliptic graphs in polynomial time

Recently, a new set of multigraph parameters was defined, called "gonalities". Gonality bears some similarity to treewidth, and is a relevant graph parameter for problems in number theory and multigraph algorithms. Multigraphs of gonality 1 are trees. We consider so-called "hyperelliptic graphs" (multigraphs of gonality 2) and provide a safe and complete sets of reduction rules for such multigraphs, showing that for three of the flavors of gonality, we can recognize hyperelliptic graphs in O(n log n+m) time, where n is the number of vertices and m the number of edges of the multigraph.

==> plaatjes/rule10.tex <==
\begin{tikzpicture}
	\cirkelsEnPijlGeenPad
	\lus{groen}{4.25}{.375}
	\lus{groen}{4.25}{-.375}
	\node[vertexx] (u) at (1.25,.375) {};
	\node[vertexx] (v) at (1.25,-.375) {};
	\node[vertexx] (u') at (4.25,0.375) {};
	\node[vertexx] (v') at (4.25,-.375) {};
	\draw[edge] (u) to [relative, out=40, in=140] (v);
	\draw[edge] (v) to [relative, out=40, in=140] (u);
\end{tikzpicture} 

==> plaatjes/rule6.tex <==
\begin{tikzpicture}
	\cirkelsEnPijlGeenPad
	\lus{groen}{0}{0}
	\lus{groen}{4.25}{.375}
	\lus{groen}{4.25}{-.375}
	\node[vertexx] (w1) at (1.25,.375) {};
	\node[vertexx] (w2) at (1.25,-.375) {};
	\node[vertexx] (v) at (0,0) {};
	\draw[edge] (v)--(w1) (w2) -- (v);
	\node[vertexx] (u') at (4.25,0.375) {};
	\node[vertexx] (v') at (4.25,-.375) {};
\end{tikzpicture} 

==> plaatjes/sdgon/eindGrafen.tex <==
\begin{figure}
		\centering
		\begin{tikzpicture}
		\node (H1) at (-1.5,.6) {$H_1$};
		\node (H2) at (.5,.6) {$H_2$};
		\node (H3) at (3.5,.6) {$H_3$};
		\lus{rood}{2}{0}
		\node[vertexx] (v) at (-1, 0) {};
		\node[vertexx] (u) at (2, 0) {};
		\node[vertexx] (a) at (4,0) {};
		\node[vertexx] (b) at (5,0) {};
		\draw[rood] (a) -- (b);
		\end{tikzpicture}
		\caption{The graphs that can remain after applying the algorithm to a graph with stable divisorial gonality 2.}  \label{fig:sdgonEndGraphs}
	\end{figure}
